Selecting Continuous Life-Like Cellular Automata for Halting Unpredictability: Evolving for Abiogenesis

Substantial efforts have been applied to engineer CA with desired emergent properties, such as supporting gliders. Recent work in continuous CA has generated a wide variety of compelling bioreminiscent patterns, and the expansion of CA research into continuously-valued domains, multiple channels, and higher dimensions complicates their study. In this work we devise a strategy for evolving CA and CA patterns in two steps, based on the simple idea that CA are likely to be complex and computationally capable if they support patterns that grow indefinitely as well as patterns that vanish completely, and are difficult to predict the difference in advance. The second part of our strategy evolves patterns by selecting for mobility and conservation of mean cell value. We validate our pattern evolution method by re-discovering gliders in 17 of 17 Lenia CA, and also report 4 new evolved CA and 1 randomly evolved CA that support novel evolved glider patterns. The CA reported here share neighborhood kernels with previously described Lenia CA, but exhibit a wider range of typical dynamics than their Lenia counterparts. Code for evolving continuous CA is made available under an MIT License (https://github.com/rivesunder/yuca).

==> old_bibliography.tex <==

\begin{thebibliography}{99}

\bibitem{rafler2011}
S. Rafler, ``Generalization of Conway's `Game of Life' to a continuous domain - SmoothLife,'' arXiv:1111.1567, Dec. 2011, Accessed: Nov. 26, 2021. [Online]. Available: \url{https://arxiv.org/abs/1111.1567}

\bibitem{chan2019}
B. W.-C. Chan, ``Lenia - Biology of Artificial Life,'' ComplexSystems, vol. 28, no. 3, pp. 251-286, Oct. 2019, doi: 10.25088/ComplexSystems.28.3.251.

\bibitem{chan2020}
B. W.-C. Chan, ``Lenia and Expanded Universe,'' The 2020 Conference on Artificial Life, pp. 221-229, 2020, doi: \url{10.1162/isal_a_00297}.

\bibitem{eppstein2010}
D. Eppstein, ``Growth and Decay in Life-Like Cellular Automata,'' arXiv:0911.2890, pp. 71-97, 2010, doi: \url{10.1007/978-1-84996-217-9_6}.

\bibitem{wolfram1984}
S. Wolfram, ``UNIVERSALITY AND COMPLEXITY IN CELLULAR AUTOMATA,'' p. 35.

\bibitem{conwaylifeforum} 
``List of the Turing-complete totalistic life-like CA" (discussion thread) at the ConwayLife.com forums \url{https://web.archive.org/web/20211031150255/https://www.conwaylife.com/forums/viewtopic.php?t=&p=102550}

\bibitem{cook2004}
M. Cook, ``Universality in Elementary Cellular Automata,'' Complex Systems, p. 40, 2004.

\bibitem{metacell}

\url{https://b3s23life.blogspot.com/2006_09_01_archive.html}


\bibitem{hansen2014}
N. Hansen. The CMA Evolution Strategy: A Tutorial. 2005. ffhal-01297037f \url{https://arxiv.org/abs/1604.00772}

\bibitem{evans2001}
K. M. Evans, Larger than Life: Digital Creatures in a Family of Two-Dimensional Cellular Automata, Discrete Mathematics \& Theoretical Computer Science, vol. DMTCS Proceedings vol. AA,..., no. Proceedings, p. 2288, Jan. 2001, doi: 10.46298/dmtcs.2288.


\bibitem{pivato2007}
M. Pivato, ``RealLife: the continuum limit of Larger Than Life cellular automata,'' Theoretical Computer Science, vol. 372, no. 1, pp. 46-68, Mar. 2007, doi: 10.1016/j.tcs.2006.11.019.

\bibitem{eppstein2010}
D. Eppstein, ``Growth and Decay in Life-Like Cellular Automata,'' arXiv:0911.2890, pp. 71–97, 2010, doi: 10.1007/978-1-84996-217-9\_6.

\bibitem{wolfram1984}
S. Wolfram, ``UNIVERSALITY AND COMPLEXITY IN CELLULAR AUTOMATA,'' p. 35.

\bibitem{cook2004}
M. Cook, ``Universality in Elementary Cellular Automata,'' Complex Systems, p. 40, 2004.

\bibitem{carter1983}
B. Carter. ``The anthropic principle and its implications for biological evolution,'' Phil. Trans. R. Soc. Lond. A, vol. 310, no. 1512, pp. 347–363, Dec. 1983, doi: 10.1098/rsta.1983.0096.

\bibitem{carter1974}
B. Carter, ``Large Number Coincidences and the Anthropic Principle in Cosmology,'' in Confrontation of Cosmological Theories with Observational Data, M. S. Longair, Ed. Dordrecht: Springer Netherlands, 1974, pp. 291–298. doi: 10.1007/978-94-010-2220-0\_25.

\bibitem{gardner1970}
M. Gardner. ``Mathematical Games - The fantastic combinations of John Conway’s new solitaire game `life' 223 (October 1970): 120-123.


\bibitem{langton1990}
C. G. Langton, ``Computation at the edge of chaos: Phase transitions and emergent computation,'' Physica D: Nonlinear Phenomena, vol. 42, no. 1–3, pp. 12–37, Jun. 1990, doi: 10.1016/0167-2789(90)90064-V.


\bibitem{packard1984}
N. H. Packard and S. Wolfram, ``Two-dimensional cellular automata,'' p. 46. 1984

\bibitem{kingma2017}
D. P. Kingma and J. Ba, ``Adam: A Method for Stochastic Optimization,'' arXiv:1412.6980 [cs], Jan. 2017, \url{https://arxiv.org/abs/1412.6980}

\bibitem{stanley2007}
K. O. Stanley, ``Compositional pattern producing networks: A novel abstraction of development,'' Genet Program Evolvable Mach, vol. 8, no. 2, pp. 131–162, Jun. 2007, doi: 10.1007/s10710-007-9028-8.

\bibitem{toffoli1987}
T. Toffoli and N. Margolus, Cellular Automata Machines: A New Environment for Modeling. The MIT Press, 1987. doi: 10.7551/mitpress/1763.001.0001.

\bibitem{turing1936}
Turing, Alan Mathison. ``On computable numbers, with an application to the Entscheidungsproblem.'' J. of Math 58.345-363 (1936): 5.
%[17]``Turing_Paper_1936.pdf.'' 


\bibitem{rendell2011}
P. Rendell, ``A Universal Turing Machine in Conway's Game of Life,'' in 2011 International Conference on High Performance Computing \& Simulation, Istanbul, Turkey, Jul. 2011, pp. 764–772. doi: 10.1109/HPCSim.2011.5999906.


\end{thebibliography}
